Towards Adapting ImageNet to Reality: Scalable Domain Adaptation with Implicit Low-rank Transformations

Images seen during test time are often not from the same distribution as images used for learning. This problem, known as domain shift, occurs when training classifiers from object-centric internet image databases and trying to apply them directly to scene understanding tasks. The consequence is often severe performance degradation and is one of the major barriers for the application of classifiers in real-world systems. In this paper, we show how to learn transform-based domain adaptation classifiers in a scalable manner. The key idea is to exploit an implicit rank constraint, originated from a max-margin domain adaptation formulation, to make optimization tractable. Experiments show that the transformation between domains can be very efficiently learned from data and easily applied to new categories. This begins to bridge the gap between large-scale internet image collections and object images captured in everyday life environments.

==> mmdt.tex <==
\section{Max-Margin Domain Transform}

In this paper, we show how to extend transform-based domain adaptation towards large-scale settings. In particular, we show how to efficiently solve the max-margin domain transform (MMDT) learning approach~\cite{Hoffman13:ELD}. In a supervised domain adaptation setting, we are given source training examples $\dataset = \left\{ (\inputsingle_i, \labelsingle_i) \right\}_{i=1}^\noe$ and target training examples $\dadataset = \left\{ (\dainputsingle_j, \dalabelsingle_j) \right\}_{j=1}^{\tilde{\noe}}$. Our goal is then to learn linear one-vs-all classification models $f_k(\inputsingle) = \hyperplane_k^T \inputsingle$, which have shown to be suitable for large-scale settings~\cite{} and also comparable to non-linear models with explicit kernel embeddings~\cite{Vedaldi10:EAK}. 

The key idea of MMDT is to learn a linear transformation $\datransform \dainputsingle$ of the target training examples into the source domain, such that the transformed data points are correctly classified. This goal can be expressed as a combined SVM problem, where hyperplane parameters $\hyperplane_k$ for each class $k$ and the transformation matrix $\datransform$ are learned jointly:
\optimizationProblem{eq:mmdt}{\min}
                    {\datransform, \{ \hyperplane_k, \vec{\eta}^k, \vec{\xi}^k \}}
                    {\frac{1}{2} \| \datransform \|^2_F + \frac{1}{2} \sum\limits_{k=1}^K \| \hyperplane_k \|^2_2\\&&&\quad + C \sum\limits_{i,k} \left( \xi^k_i \right)^p + \tilde{C} \sum\limits_{j,k} \left( \eta^k_j \right)^p }
                    { \labelsingle^k_i \left( \hyperplane_k^T  \inputsingle_i \right) \geq 1 - \xi_i^k \quad \forall i,k\\&&&
                      \dalabelsingle^k_j \left( \hyperplane_k^T \datransform \dainputsingle_j  \right) \geq 1 - \eta_j^k \quad \forall j,k\\&&&
                      \xi^k_i \geq 0 \quad \forall i,k\\&&&
                      \eta^k_j \geq 0 \quad \forall j,k
                      }
The indices $1 \leq i \leq \noe$, $1 \leq j \leq \tilde{\noe}$ and $1 \leq k \leq K$ enumerate the source domain examples, target domain examples, and classes, respectively. The parameter $p \in \{1,2\}$ determines whether L1-SVM or L2-SVM is used~\cite{Hsieh08:DCD}. 

For optimization, \cite{Hoffman13:ELD} suggests using a block-wise coordinate descent optimization in  $\datransform$ and $\{ \hyperplane_k \}$. 
Optimizing with respect to the hyperplane parameters is straightforward and can be done in the linear case by first applying the transformation $\datransform$ and solving a soft-margin SVM problem, for which many large-scale solvers are available~\cite{Hsieh08:DCD}. The block-wise coordinate descent strategy is also beneficial, because we are normally confronted with large source domain datasets. Optimizing for $\datransform$ with fixed linear classifiers only requires access to the target examples and $\{ \hyperplane_k \}$, which summarize the source training data.
However, learning $\datransform$ is still an expensive operation with several thousands of high-dimensional target feature vectors.

